Group cohesion under asymmetric voting behaviors

Cohesion plays a crucial role in achieving collective goals, promoting cooperation and trust, and improving efficiency within social groups. To gain deeper insights into the dynamics of group cohesion, we have extended our previous model of noisy group formation by incorporating asymmetric voting behaviors. Through a combination of theoretical analysis and numerical simulations, we have explored the impact of asymmetric voting noise, the attention decay rate, voter selection methods, and group sizes on group cohesion. For a single voter, we discovered that as the group size approaches infinity, group cohesion converges to $1/(R+1)$, where $R$ represents the ratio of asymmetric voting noise. Remarkably, even in scenarios with extreme voting asymmetry ($R \to \infty$), a significant level of group cohesion can be maintained. Furthermore, when the positive or negative voter's voting noise surpasses or falls below the phase transition point of $R_c=1$, a higher rate of attention decay can lead to increased group cohesion. In the case of multiple voters, a similar phenomenon arises when the attention decay rate reaches a critical point. These insights provide practical implications for fostering effective collaboration and teamwork within growing groups striving to achieve shared objectives.

==> temp.tex <==
Where the two terms correspond to $\sigma_i = + 1$ ($i$ is fit) and $\sigma_i = - 1$ ($i$ is unfit), respectively. For the dictatorship case, only the founder members are allowed to evaluate, so $i = 0$ and $P(t) = W(0) = 1 - \alpha$. Cohesion is then given by

% \begin{equation}
%     \overline{C(N,N_0,\alpha)_{DS}} = (1 - \alpha) + \frac{\alpha N_0}{N}
% \end{equation}

% As $N \to \infty$, group cohesion thus approaches $1 - \alpha$, i.e., it decreases linearly with noise.
% For the uniform case, the t-th admitted member can be evaluated by a random group member $i$ with $i < t$; 

% which is a recursive equation for $P(t)$ with the initial condition
% $P(0) = 1$. Eq. (4) can be rearranged as



% which can be solved analytically. 

% When $\alpha = 0$,$\overline{C(N,N_0,\alpha,\beta}=1$ for any $N$ and $N_0$, as only fit candidates can be admitted.However, the expected cohesion decreases fast with $\alpha+\beta$ and is always lower than that of the dictatorship case .
% |
% |
% |

% To study the impact of introducing social capital in the model, we now consider choosing the evaluating member by the classical PA mechanism. To this end, we keep an activity counter, $k$, for all group members. This counter increases by 1 for each involvement in the admission of a new member.Without loss of generality, we set the initial activity counter to $a_0 := N_0 - 1$ and 1 for all founder members and the later admitted group members, respectively (when $N0 = 1$, we set $a_0 = 1$ to avoid zero counter of the sole founder member).
% The probability to choose a member is assumed to be directly proportional to the activity counter. Using the continuum approximation for the dynamics of the activity counter,we can write

% \begin{equation}
%     k_i(t+1) = k_i(t)+\frac{k_i(t)}{2t+N_0a_0}
% \end{equation}

% where the second term on the rhs reflects the PA selection mechanism.
% Analogously to Eq. (4), the probability that the t-th admitted member is fit for the group, $P(t)$, for the PA case reads

% \begin{equation}
%     P(t+1) = N_0\frac{W(0)k_0(t)}{2t+N_0a_0}+\sum_{i=1}^t\frac{W(i)k_i(t)}{2t+N_0a_0}
% \end{equation}

% where $W(i)$ is defined by Eq. (2). With the solution of Eq. (8)
% and the initial condition $P(0) = 1$, Eq. (9) can be rearranged
% to a simpler form (similar to Eq. (5))

% \begin{equation}
%     P(t+1)=(1-\frac{\alpha+\beta}{2t+N_0a_0})P(t)+\frac{\beta}{2t+N_0a_0}
% \end{equation}

% Similarly to the uniform case, the expected group cohesion is obtained by averaging the obtained $P(t)$ over $t = 0, ... , N - N_0$(again assigning weight $N_0$ to $t = 0$). We see  that the expected cohesion still decreases rapidly with $\alpha+\beta$, yet it differs from the uniform case. When $N \to \infty$ and $N_0$ is fixed, the leading contribution to cohesion is

% \begin{equation}
%     \overline{C(N,N_0,\alpha,\beta)_{PA}}=\frac{\beta}{\alpha+\beta}+\frac{\alpha}{\alpha+\beta}\frac{\Gamma(\frac{N_0a_0}{2})\Gamma(\frac{N_0a_0-\alpha-\beta}{2}+t)}{\Gamma(\frac{N_0a_0-\alpha-\beta}{2})\Gamma(\frac{N_0a_0}{2}+t)}
% \end{equation}

% When $N_0$ is fixed and$ N \gg N_0$,Eq. (11) implies

% \begin{equation}
%     \overline{C(N,N_0,\alpha,\beta)_{PA}} \approx N^{\frac{-\alpha-\beta}{2}}\frac{\Gamma(\frac{N_0a_0}{2})}{\Gamma(\frac{N_0a_0-\alpha-\beta}{2})}
% \end{equation}

% We find that group cohesion in the PA case is not only higher than in the uniform case, it also decays with $N$ slower: the scaling exponent is $\frac{\alpha+\beta}{2}$ instead of $\alpha+\beta$. This higher robustness is due to preferential attachment effectively giving more power to early group members who, on average, are more likely to be fit than group members who join the group later. At the same time, the limit cohesion remains unchanged: as the group grows, its cohesion approaches the cohesion of a random group.

% The advantages of our approach lie in the introduction of a unified formal framework to represent the 

% \section{Discussion}





% evolution of opinions in different groups with non-Markovian properties.

% Our results have the following main implications: Firstly, in the UC and PA scenarios, unlike having equal discriminatory abilities as all groups, even if one party is only a small fraction of noise, the level of disagreement increases as the proportion of noise from the other party increases. Interestingly, as more individuals start voting, the impact of different group noise proportions on the level of disagreement diminishes.


% When there are more than one voters ($m > 1$), admission is granted only if all votes are positive. Let's first consider the case of $m = 2$, represented by voters $i$ and $j$. Therefore, the probability of an admitted member being fit can be expressed as:

% \begin{equation}
%     W_{ij} = \frac{W(i)W(j)}{W(i)W(j)+[1-W(i)][1-W(j)]}
% \end{equation}

% In the case of multiple-person voting, group cohesion does not decrease as the rate of decline in judgment increases. On the contrary, it starts to increase after reaching a critical point and eventually converges to a stable point.This is because with the increase in the rate of decay, the judgment capability of older members (i.e., those who joined the group earlier) tends to approach a random level, thereby losing the advantage of their initial judgment capability.


% In the given scenario, we investigate the relationship between the proportion of fit people and parameter b in a voting process. Initially, considering the case where only one person votes, we observe a gradual decrease in the proportion of fit people as the value of b increases. This implies that as the influence of the individual voter strengthens, the likelihood of selecting option-fit people diminishes.

% However, the dynamics change significantly when multiple individuals participate in the voting process. Through our analysis, we have identified a critical point known as the phase transition point, beyond which the system exhibits a remarkable shift in behavior. Upon reaching this transition point, characterized by a specific threshold value of $b$, we observe a notable increase in the proportion of fit people as b continues to increase.

% These findings suggest that the collective decision-making process, when influenced by the votes of multiple individuals, can lead to a significant alteration in the outcome compared to when only one person is involved. The occurrence of the phase transition indicates a qualitative change in the system dynamics, indicating the emergence of consensus or a dominant choice as the influence of the participants grows.

% Further investigation and analysis are required to elucidate the underlying mechanisms driving this phase transition phenomenon and to explore its implications in various contexts, such as social decision-making, opinion dynamics, and collective behavior. Understanding the factors that contribute to this transition can provide valuable insights into the dynamics of complex systems and enhance our comprehension of the underlying principles governing collective decision-making processes.



% Our research findings demonstrate that the number of participants involved in the assessment of new candidates plays a crucial role in determining the cohesion of the entire group. Under the condition of fixed judgment ability for non-dominant party members, we observed that increasing the number of voters is an effective way to enhance cohesion before the crossover point while reducing the number of voters is found to strengthen group cohesion after the crossover point. In contrast, under the condition of fixed judgment ability for dominant party members, the cohesion of the group remains within a fixed range regardless of the judgment ability of non-dominant party members.

% These findings emphasize the importance of the number of evaluators in group cohesion and provide a deeper understanding of group decision-making and behavior. Further research can explore the relationship between the number of evaluators and group cohesion in different contexts, as well as investigate approaches to optimize decision-making effectiveness and collaborative capabilities within groups. This has significant implications for improving decision quality and performance in organizations and social systems.




% We further considered the scenario of evaluators having memory in their voting behavior. Under the condition of individual evaluator voting, increasing the evaluation parameter has different trends on group cohesion depending on the evaluation mechanism. Specifically, under the UC (Unique Memory and Cooperative Memory) mechanism, as one evaluation parameter remains fixed, increasing the other evaluation parameter gradually decreases group cohesion. However, under the PA (Expert Memory and Average Memory) mechanism, the opposite trend is observed. Moreover, when alpha/beta is fixed at specific values, regardless of the increase in parameter b, group cohesion tends to converge to a stable level. Before the crossover point, group cohesion shows an increasing trend with the increase of parameter b, while after the crossover point, it exhibits a decreasing trend with the decrease of parameter b.

% These findings provide a deeper understanding of the impact of evaluators' memory-based voting on group cohesion and reveal dynamic variations under different evaluation mechanisms. Further research can explore the effects of evaluators' memory on group decision-making and collaboration, providing valuable guidance for decision processes in organizations and social systems to enhance overall performance and decision effectiveness.



% In the context of multi-person voting, when alpha is fixed, the group cohesion corresponding to different values of b tends to stabilize as beta increases. Building upon this observation, we further investigated the scenario where beta approaches zero, i.e., when $\alpha/\beta$ tends to infinity. As b increases, a phase transition in group cohesion is observed.

% This research reveals the impact of evaluation parameters on group cohesion in multi-person voting and uncovers the phase transition phenomenon under specific conditions. Further research can delve into the relationship between alpha and beta and explore the effects of different voting mechanisms on group behavior and decision-making, providing a deeper understanding of collective decision-making and social collaboration. These findings are of significant importance for comprehending decision processes and dynamic behavior within organizations and social systems.




% \begin{figure}[htp]
%     \centering
%     \includegraphics[width=12cm]{Figs/alpha_beta.png}
%     \caption{Unknown}
%     \label{fig:unknown_1}
% \end{figure}
% \begin{equation}
%     k(i,t) = 1+\frac{1}{N_0+i-1}+...+\frac{1}{N_0+t-1} = 1 + ln(\frac{t}{i})
% \end{equation}

% Then Eq.\ref{lab-W} can be expressed as

% \begin{equation}
%     W(i,t) = P(i)\Big(1-\alpha(i,t)\Big) + \Big(1-P(i)\Big)\beta(i,t).
% \end{equation}

% Firstly, we will explore the use of the UC mechanism for selecting evaluators. Then Eq.\ref{lab-PPP} become

% % Where $b$ is the slope coefficient, the degree of control on judgment 

% \begin{equation}
%     \label{lab-P1}
%     P(t+1) = \frac{N_0}{t+N_0}W(0,t) + \frac{1}{t+N_0}\sum_{i=1}^{t}W(i,t)
% \end{equation}

% % \begin{equation}
% %     \label{lab-P1}
% %     (t+N_0)P(t+1) - (t+N_0-1)P(t) = N_0\left [ W(0,t) - W(0,t-1) \right ] +W(t,t) + \sum_{i=1}^{t-1}\left [ W(i,t)-W(i,t-1) \right ] 
% % \end{equation}

% % in this equation

% % \begin{equation}
% %     
% %     (t+N_0)\left [ P(t+1) - P(t) \right ] = N_0 \left [ W(0,t) - W(0,t-1) \right ] - (\alpha+\beta)P(t) + \beta + \sum_{i=1}^{t-1}\left [ W(i,t)-W(i,t-1) \right ] 
% % \end{equation}

% when $t \to \infty$ then $P(t+1)-P(t) = 0$, Eq.\ref{lab-P1} become

% \begin{equation}
%     P(\infty) = \frac{\beta + N_0\Big(\alpha(0,t-1)-\alpha(0,t)\Big) + \sum_{i=1}^{t-1}\left [ W(i,t)-W(i,t-1) \right ] }{\alpha+\beta}
% \end{equation}

% Next, we will explore the use of the PA mechanism for selecting evaluators.then Eq.\ref{lab-PPP} become

% \begin{equation}
%     \label{lab-P2}
%     P(t+1) = \frac{N_0}{2t+N_{0}a_{0}}W(0,t)k(0,t) + \frac{1}{2t+N_{0}a_{0}}\sum_{i=1}^{t}W(i,t)k(i,t)
% \end{equation}

% % \begin{equation}
% %     \label{lab-P}
% %     (2t+N_0(N_0-1))P(t+1) - (2t+N_0(N_0-1)-2)P(t) = N_0\left [ W(0,t)k(0,t) - W(0,t-1)k(0,t-1) \right ] +W(t,t)k(t,t) + \sum_{i=1}^{t-1}\left [ W(i,t)k(i,t)-W(i,t-1)k(i,t-1) \right ] 
% % \end{equation}

% when $t \to \infty$ then $P(t+1)-P(t) = 0$, Eq.\ref{lab-P2} become

% \begin{equation}
%     P(\infty) = \frac{\beta + N_0\Big(\alpha(0,t-1)-\alpha(0,t)\Big) +\sum_{i=1}^{t-1}\left [ W(i,t)k(i,t)-W(i,t-1)k(i,t-1) \right ] }{1+\alpha+\beta}
% \end{equation}


% In this section, we introduce a non-Markovian decision mechanism, where the judgment capability of agents depends on their accumulated experience, represented by the number of decision-making instances they have undergone. This accumulated experience can be regarded as the "decision-making expertise" of agents and has a significant impact on their future decision-making. By considering the agents' decision-making expertise, we can gain a better understanding and explanation of their decision-making behavior in specific contexts and delve into the influence of the non-Markovian nature of the decision-making process on the overall system behavior. The introduction of this concept provides us with a new perspective to comprehensively study and comprehend the decision-making processes in complex systems.

% \begin{equation}
%     \left<  k \right> = \frac{2M}{N} = \frac{2mN}{N} = 2m
% \end{equation}

% when $t \to \infty$,

% \begin{equation}
% \left \{
%  \begin{aligned}
%         \alpha (\infty)_{mean} = \alpha + \left(\frac{1}{2} - \alpha\right)\tanh \left[b\left(\left<  k \right>-1\right)\right], \\
%             \beta (\infty)_{mean} = \beta + \left(\frac{1}{2} - \beta\right)\tanh \left[b\left(\left<  k \right>-1\right)\right].
%  \end{aligned}
%  \right.
% \end{equation}

% then

% \begin{equation}
%     \overline{C}(1 - \alpha (\infty)_{mean}) +\overline{C}\beta (\infty)_{mean} = \overline{C}
% \end{equation}

% so

% \begin{equation}
%     \overline{C} = \frac{\beta + \left(\frac{1}{2} - \beta\right)\tanh \left[b\left(\left<  k \right>-1\right)\right].}{\alpha + \beta + \left(1 - \alpha - \beta\right)\tanh \left[b\left(\left<  k \right>-1\right)\right].}
% \end{equation}

% when $\alpha = \beta$,$\overline{C} = \frac{1}{2}$

% In contrast to previous studies, our research findings indicate that regardless of the magnitude of positive noise in the system, disagreements evolve with changing proportions as the team grows. Moreover, as the group size approaches infinity, disagreements gradually increase until reaching a threshold. In other words, fragmentation is inevitable in large social groups.

% Our model oversimplifies the complexity of social dynamics. While the introduced noise parameters in this study effectively represent the random factors involved in the interactions between individuals, the emergence of disagreements is a complex phenomenon influenced by numerous difficult-to-discern factors. Nonetheless, our work focuses on a specific aspect of group formation and offers a complementary explanation to existing interpretations of social fragmentation.
% Through theoretical analysis and numerical simulations, the article explores the effects of different voting parameters, selection methods, and group size on group cohesion. The study finds that under certain levels of noise, as the group expands, cohesion spontaneously decreases, even reaching critical points and undergoing phase transitions. This suggests that divergence and fragmentation are inevitable in large social groups.

% Furthermore, the study reveals that behavioral differences among individuals during the voting process (i.e., asymmetry) influence the trend of group cohesion. When individuals with initial beliefs (+1) are more accepting of candidates with opposing views (-1) (i.e., α > β), cohesion gradually decreases as the group size increases. However, when individuals with initial beliefs (+1) are less accepting of candidates with opposing views (-1) (i.e., α < β), cohesion initially decreases and then increases, ultimately converging to a stable value as the group size grows.

% Additionally, the study finds that differences in individual influence during the voting process (i.e., selection methods) also affect the trend of group cohesion. When individuals are randomly selected as voters (i.e., uniform selection), cohesion decreases with increasing group size. However, when individuals are selected as voters proportionally to their past participation in voting (i.e., preferential attachment), cohesion increases with increasing group size. This indicates that group cohesion is higher when social influence mechanisms are present.

% Moreover, the study reveals that attention decay among individuals during the voting process (i.e., non-Markovian behavior) also influences the trend of group cohesion. When individuals' attention does not decay during the voting process (i.e., b = 0), cohesion decreases with increasing group size. However, when individuals' attention decays during the voting process (i.e., b > 0), cohesion increases with increasing group size. This suggests that group cohesion is higher when memory effects are present.

